Sound Dynamic Deadlock Prediction in Linear Time

Deadlocks are one of the most notorious concurrency bugs, and significant research has focused on detecting them efficiently. Dynamic predictive analyses work by observing concurrent executions, and reason about alternative interleavings that can witness concurrency bugs. Such techniques offer scalability and sound bug reports, and have emerged as an effective approach for concurrency bug detection, such as data races. Effective dynamic deadlock prediction, however, has proven a challenging task, as no deadlock predictor currently meets the requirements of soundness, high-precision, and efficiency. In this paper, we first formally establish that this tradeoff is unavoidable, by showing that (a) sound and complete deadlock prediction is intractable, in general, and (b) even the seemingly simpler task of determining the presence of potential deadlocks, which often serve as unsound witnesses for actual predictable deadlocks, is intractable. The main contribution of this work is a new class of predictable deadlocks, called sync(hronization)-preserving deadlocks. Informally, these are deadlocks that can be predicted by reordering the observed execution while preserving the relative order of conflicting critical sections. We present two algorithms for sound deadlock prediction based on this notion. Our first algorithm SPDOffline detects all sync-preserving deadlocks, with running time that is linear per abstract deadlock pattern, a novel notion also introduced in this work. Our second algorithm SPDOnline predicts all sync-preserving deadlocks that involve two threads in a strictly online fashion, runs in overall linear time, and is better suited for a runtime monitoring setting. We implemented both our algorithms and evaluated their ability to perform offline and online deadlock-prediction on a large dataset of standard benchmarks.

==> algo-online_full.tex <==
%!TEX root = main.tex

\small
\begin{algorithm*}[H]
% \BlankLine
\begin{multicols}{2}
\myfun{\init{}}{
	\ForEach{$t \in \threads{}$ $\cdot$}{
		$\Cc_t$ := $\bot$
	}
	\ForEach{$x \in \vars{}$ $\cdot$}{
		$\LW_x$ := $\bot$
	}
	\ForEach{$\lk \in \locks{}$ $\cdot$}{
		$\gId_\lk$ := $0$
	}
	\ForEach{$t_1 {\neq}t_2 \in \threads{}, \lk_1 {\neq} \lk_2 \in \locks{}$}{
		$\view{\Ii}{}{\tuple{t_1, \lk_1, t_2, \lk_2}}$ := $\bot$ \;
		\ForEach{$t \in \threads{}, \lk \in \locks{}$}{
			$\view{\AcqLst}{t, \lk}{\tuple{t_1, \lk_1, t_2, \lk_2}}$ := $\epsilon$
		}
	}
	\ForEach{$u \in \threads{}$}{
		\ForEach{$t\in \threads{}, \lk_1, \lk_2 \in \locks{}$}{
			$\view{\DPLst}{t, \lk_1, \lk_2}{\tuple{u}}$ := $\epsilon$
		}
	}
}
\BlankLine
% {\tiny \tcp{$Lst$ is a list of triplets $(g, C, C')$ in increasing order of $C$}}
% {\tiny \tcp{Returns the last element $(g_{\max}, C_{\max}, C'_{\max})$ s.t. $C_{\max} \cle U$}}
% {\tiny \tcp{Removes all other elements $(g,C, C')$ from $Lst$ with $C \cle U$}}
\myfun{\maxLB{$U$, $Lst$}}{
	$(g_{\max}, C_{\max}, C'_{\max})$ := $(0, \bot, \bot)$ \; 
	\While{$\NOT\, \isEmpty{Lst}$}{
		$(g, C, C')$ := $\first{Lst}$ \;
		\If{$C \cle U$}{
			$(g_{\max}, C_{\max}, C'_{\max})$ := $(g, C, C')$
		}
		\Else{
			\Break
		}
		$\removeFirst{Lst}$
	}
	\Return $(g_{\max}, C_{\max}, C'_{\max})$
}

\BlankLine

\myfun{\fixpoint{$I$, $\tuple{t_1, \lk_1, t_2, \lk_2}$}}{
	\Repeat{$I$ does not change}{
		\ForEach{$\lk \in \locks{}$}{
			\ForEach{$t \in \threads{}$}{
				($g_{\lk, t}, C_{\lk, t}, C'_{\lk, t}$) := 
				\maxLB{$I$, $\view{\AcqLst}{t, \lk}{\tuple{t_1, \lk_1, t_2, \lk_2}}$} \;
			}
			$t_{\max}$ := argmax$_{t \in \threads{}}\set{g_{\lk, t}}$ \;
			$I$ := $I \mx \bigsqcup_{t \neq t_{\max} \in \threads{}} C'_{\lk, t}$	
		}
	}
	\Return $I$
}

\myfun{\checkDeadlock{$Lst$, $I$, $\tuple{t_1, \lk_1, t_2, \lk_2}$}}{
	\While{$\NOT\, \isEmpty{Lst}$}{
		($C_{\prev{}}, C$) := $\first{Lst}$ \;
		$I$ := \fixpoint{$I \mx C_{\prev{}}$, $\tuple{t_1, \lk_1, t_2, \lk_2}$} \;
		\If{$C \not\cle I$}{ \linelabel{check-containment}
			\declare `Deadlock' \;
			\Break
		}
		$\removeFirst{Lst}$
	}
	\Return $I$
}

\myhandler{\rdhandler{$t$, $x$}}{
	$\Cc_t$ := $\Cc_t \mx \LW_x$ \linelabel{clkrd}
}

\myhandler{\wthandler{$t$, $x$}}{
	$\LW_x$ := $\Cc_t$ \linelabel{clkwt};\\
	$\Cc_t$ := $\Cc_t[t \mapsto \Cc_t(t)+1]$
}

\myhandler{\acqhandler{$t$, $\lk$}}{
	$C_{\prev{}}$ := $\Cc_t$ \;
	$\Cc_t$ := $\Cc_t[t \mapsto \Cc_t(t)+1]$\\ $\gId_\lk$ := $\gId_\lk + 1$ \linelabel{clkacq}\;
	\ForEach{$t_1, t_2 \in \threads{}, \lk_1, \lk_2 \in \locks{}$}{
		$\addLst{\view{\AcqLst}{t, \lk}{\tuple{t_1, \lk_1, t_2, \lk_2}}}{$(\gId_\lk, \Cc_t, \bot)$}$
	}
	\ForEach{$u\in \threads{}$, $\lk' \in \lheld{}$}{
		$\addLst{\view{\DPLst}{t, \lk, \lk'}{\tuple{u}}}{($C_{\prev{}}$, $\Cc_t$)}$
	}
	\ForEach{$u \neq t \in \threads{}$, $\lk' \in \lheld{}$}{
		$I$ := $\view{\Ii}{}{\tuple{u, \lk' t, \lk}} \mx C_{\prev{}}$ \;
		$\view{\Ii}{}{\tuple{u, \lk' t, \lk}}$ := \checkDeadlock{$\view{\DPLst}{u, \lk', \lk\,}{\tuple{t}}$, $I$, $\tuple{u, \lk' t, \lk}$}
	}

}

\myhandler{\relhandler{$t$, $\lk$}}{
	$\Cc_t$ := $\Cc_t[t \mapsto \Cc_t(t)+1]$ \linelabel{clkrel} \;
	\ForEach{$t_1, t_2 \in \threads{}, \lk_1, \lk_2 \in  \locks{}$}{
		$\updateRel{\lst{\view{\AcqLst}{t, \lk}{\tuple{t_1, \lk_1, t_2, \lk_2}}}}{$\Cc_t$}$
	}
}


\end{multicols}
% \vspace*{0.25cm}
\normalsize
\caption{$\SyncPDOnline$.}
\algolabel{online}
\end{algorithm*}
\normalsize

==> app-algo.tex <==
%!TEX root = main.tex

\section{Details of Algorithms}

%\subsection{Verifying Abstract Deadlock Patterns}
%\applabel{verify-abstract-patterns}

%Given an abstract deadlock pattern of length $k \geq 2$,
%there can be $O(\NumEvents^k)$ instantiations of it,
%giving a naive enumerate-and-check algorithm running 
%in time $O(\NumThreads\cdot\NumEvents^{k+1})$.
%Instead we exploit monotonicity properties of 
%the sync-preserving closure (\propref{spclosure-monotone})
%and instantiations of an abstract pattern (\corref{pattern-monotone}) 
%that allow for an \emph{incremental}
%algorithm that iteratively checks successive instantiations
%of a given abstract deadlock pattern, while still spending total $O(\NumEvents\cdot \NumThreads)$ time.
%% , i.e., the running time is linear in $\NumEvents$, which is the dominating parameter.
%The first observation allows us to re-use a prior
%computation when checking later deadlock patterns.
%
%% We first observe that the sync-preserving closure is monotonic
%% with respect to the thread-order, and thus, when computing closure
%% of later events, one can avoid re-computation.
%\begin{restatable}{proposition}{spclosure-monotone}
%\proplabel{spclosure-monotone}
%For a trace $\tr$ and sets $S, S' \subseteq \events{\tr}$.
%If for every event $e \in S$, there is an event $e' \in S$
%such that $e \tho{\tr} e'$, then
%$\SPClosure{\tr}(S) \subseteq \SPClosure{\tr}(S')$.
%\end{restatable}
%
%%\begin{proof}
%%Follows from the definition of $\SPClosure{\tr}(S)$.
%%\end{proof}
%
%Next, we extend \propref{spclosure-monotone} to avoid redundant
%computations when a sync-preserving deadlock is not found and later deadlock patterns must be checked.
%Given two deadlock patterns
%$D_1 = e_0, \ldots, e_{k-1}$ and $D_2 = f_0, \ldots, f_{k-1}$
%of the same length $k$, 
%we say $D_1 \prec D_2$ if
%they are instantiations of a common abstract pattern $\abst{D}$
%(i.e., $D_1, D_2 \in \abst{D}$) and 
%for every $i<k$, $e_i \tho{\tr} f_i$.
%\begin{restatable}{corollary}{pattern-monotone}
%\corlabel{pattern-monotone}
%Let $\tr$ be a trace and let $D_1 = e_0, \ldots, e_{k-1}$ and 
%$D_2 = f_0, \ldots f_{k-1}$ be deadlock
%patterns of size $k$ in $\tr$ such that $D_1 \prec D_2$.
%Let $S_1 = \set{e_0, \ldots, e_{k-1}}$ and $S_2 = \set{f_0, \ldots, f_{k-1}}$.
%If $\SPClosure{\tr}(\prev{\tr}(S_1))\cap S_2 \neq \emptyset$,
%then $\SPClosure{\tr}(\prev{\tr}(S_2))\cap S_2 \neq \emptyset$.
%\end{restatable}
%
%The algorithm for checking if an abstract deadlock 
%pattern contains a sync-preserving instantiation
%is presented in~\algoref{abstract-pattern}.
%At a high level, it iterates over the sequences $F_0, \ldots, F_{k-1}$ of 
%acquires (one for each abstract acquire) in trace order.
%For this, the algorithm maintains
% indices $i_0, \ldots, i_{k-1}$ that point to entries in $F_0, \ldots, F_{k-1}$.
%At each step, it determines whether the current
%deadlock pattern $D = e_0, \ldots, e_{k-1}$
%by computing the sync-preserving closure
%of the predecessors of the deadlock pattern, and checks
%if it is disjoint from the deadlock.
%If so, it terminates.
%Otherwise, it looks for the next eligible deadlock,
%which it determines based on \corref{pattern-monotone}.
%In particular, it advances the pointer $i_j$
%all the way until an entry which is outside of the
%closure computed so far.
%Also observe that the timestamp $T$ of the closure
%computed in an iteration is being used in later iterations;
%this is a consequence of \propref{spclosure-monotone}.
%Further, we ensure that the list of acquires $\AcqLst_{t, \lk}$
%used in the function \fixpoint (\algoref{compute-closure})
%be reused across iterations, and not need be
%re-assigned to the original list of all acquire events;
%correctness of this optimization follows from~\propref{spclosure-monotone}.
%Let us now calculate the running time for this algorithm.
%Each of the $\AcqLst_{t, \lk}$ in \fixpoint is traversed
%at most once. 
%Next, each element of the sequences $F_0, \ldots, F_{k-1}$
%is also traversed atmost once.
%For each of these acquires, the algorithm spends $O(\NumThreads)$
%time for vector clock updates.
%The total time required is thus $O(\NumEvents \cdot \NumThreads)$.
%This concludes the proof of \lemref{abstract-pattern-linear-time}.

\subsection{The Online $\SyncPDOffline$ Algorithm}
\applabel{app_online}
%\seclabel{app_online}
\Andreas{We can consider bringing this in the main paper. We should have space now. Some reviewers requested this, and it does make the paper self contained.}
In this section we give a detailed pseudocode description of the online $\SyncPDOffline$ algorithm (\algoref{online}).
\input{algo-online_full}

==> app-exp.tex <==
%!TEX root = ./main.tex

\section{Further Experiments}
%\seclabel{app_experiments}
\applabel{app_experiments}

For the sake of completeness, here we report on a small experimental comparison with the SMT-based tool Dirk~\cite{Kalhauge2018}.
As the complexity of Dirk is polynomial (due to SMT solving), it uses windowing to examine segments of a large trace.
In our experiments we set a window size of 1.5K and timeout of $1$ hour.
Finally, our experiments were run on a subset of our dataset, as we faced technical challenges in executing Dirk on some benchmarks.
We nevertheless ensured that all tools were executed on identical inputs.
\cref{tab:expr-results-dirk} shows the obtained results.
We confirm that Dirk takes extremely long to complete even this subset and fails to report deadlocks on larger instances due to timeout, 
while it detects two deadlocks missed by our algorithms due to the fact that it also detects deadlocks not witnessed by correct reorderings.
In particular, Dirk reports a deadlock in the benchmarks Deadlock and Transfer.
The reordering that exposes these deadlocks changes the reads-from function so that reads observe different writes in the witness trace (which, nevertheless, write the same value as the old writes, and thus the witness is sound).
We remark that reasoning about reorderings based on values is a very intractable problem (well-known to be $\NP$-hard even for 3 threads), and thus methods based on such reasoning are not scalable.
Indeed, Dirk timed out after 1h on each benchmark that required at least 1 second in $\SyncPDOnline$ and $\SyncPDOffline$.
\input{tables/dirk_results}


==> exec_macros.tex <==
%!TEX root = main.tex

% Drawing executions. Arguments: # of threads, and execution.
\newcommand{\execution}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.5*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.5+1.3,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.5+1.3,0) -- (#1*1.5+1.3,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.5+1.3,-0.4*\y);%
  \end{tikzpicture}
}
}

\newcommand{\executioncounter}[2]{
	\scalebox{0.85}{
		\begin{tikzpicture}%
			\foreach \x in {3,...,#1}
			\node[right] at (1.5*\x+0.2,0.25) {$t_{\x}$};
			\draw (1.2,0) -- (#1*1.5+1.3,0);%
			\pgfmathsetmacro{\y}{1};%
			#2%
			\draw (1.2,0) -- (1.2,-0.4*\y);%
			\draw (#1*1.5+1.3,0) -- (#1*1.5+1.3,-0.4*\y);%
			\foreach \x in {2,...,#1}
			% \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
			\draw (1.2,-0.4*\y) -- (#1*1.5+1.3,-0.4*\y);%
		\end{tikzpicture}
	}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figev}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y} };%
\node at (#1*1.5 + 0.45,-0.4*\y) {#2};%
\pgfmathsetmacro{\y}{\y+1};
}


\newcommand{\executionlarge}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.9*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.9+1.9,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.9+1.9,0) -- (#1*1.9+1.9,-0.4*\y);%
    \foreach \x in {2,...,#1}
    % \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.9+1.9,-0.4*\y);%
  \end{tikzpicture}
}
}



% \figev arguments: thread id, event, variable/lock
\newcommand{\figevlarge}[2]{
\pgfmathsetmacro{\y}{\y+1};
\pgfmathsetmacro{\y}{\y-1};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
\node at (#1*1.9 + 0.45,-0.4*\y) {$ #2 $};%
\pgfmathsetmacro{\y}{\y+1};
}


% \figev arguments: thread id, event, variable/lock, 3rd arg = event id offset

% \newcommand{\mathresult}[1]{\pgfmathparse{#1} \pgfmathresult}
% \newcommand{\addmathresult}[1]{\pgfmathparse{2 *\mathresult{#1}} \pgfmathresult}

\newcommand{\figevoffset}[3]{
\pgfmathparse{#1}
\pgfmathsetmacro{\offset}{\pgfmathresult};
\pgfmathparse{\y+\offset}
\pgfmathsetmacro{\newindex}{\pgfmathresult};
\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\newindex}};%
\node at (#2*1.5 + 0.45,-0.4*\y) {$ $#3$ $};%
\pgfmathsetmacro{\y}{\y+1};
}

%\orderedeg{t1}{ind1}{off1}{t2}{ind2}{off2} denotes an edge from an event e1
% to an event e2 such that ei appears at indi in the trace and belongs to thread ti.
% off1 and off2 are offsets from the center.
\newcommand{\orderedge}[6]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] (#4*1.5 + 0.45 + #6, -0.4*#5);
}

% The 7th arg is the label and the 8th argument is the position
\newcommand{\orderedgewithlabel}[8]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] node[anchor=center, sloped, #8] { #7} (#4*1.5 + 0.45 + #6, -0.4*#5);
}

\newcommand{\executionnonumber}[2]{\begin{tikzpicture}%
                             \foreach \x in {1,...,#1}
                               \node[right] at (2*\x+0.5,0.25) {$t_{\x}$};
                             \draw (1.9,0) -- (#1*2+1.6,0);%
                             \pgfmathsetmacro{\z}{1};%
                             #2%
                             \draw (1.9,0) -- (1.9,-0.5*\z);%
                             \draw (#1*2+1.6,0) -- (#1*2+1.6,-0.5*\z);%
                             \foreach \x in {2,...,#1}
                               \draw (2*\x-0.3,0) -- (2*\x-0.3,-0.5*\z);%
                             \draw (1.9,-0.5*\z) -- (#1*2+1.6,-0.5*\z);%
                           \end{tikzpicture}}                    

\newcommand{\figevnonumber}[2]{\node [left] at (1.75,-0.4*\z) {};%
\node [right] at (#1*2 + 0.3,-0.5*\z) {$ #2 $};%
\pgfmathsetmacro{\z}{\z+1};}

% Drawing programs. Arguments: # of threads, and program
\newcommand{\figprogram}[2]{\begin{tikzpicture}%
                              \foreach \x in {1,...,#1}
                                \node at (2.3*\x-1.15,0.25) {$t_{\x}$};
                              \draw (0,0) -- (#1*2.3+0.6,0);% 
                              \pgfmathsetmacro{\y}{1};%
                              #2%
                              \draw (0,0) -- (0,-0.4*\y);% 
                              \draw (#1*2.3+0.6,0) -- (#1*2.3+0.6,-0.4*\y);% 
                              \draw (0,-0.4*\y) -- (#1*2.3+0.6,-0.4*\y);% 
                            \end{tikzpicture}}
% figstmt arguments: thread id, offset, statement
\newcommand{\figstmt}[3]{\node [left] at (-0.15,-0.4*\y) {\pgfmathprintnumber{\y}};%
                      \node[right] at (#1*2.3 + #2*0.3 - 2.15,-0.4*\y) {\texttt{#3}};
                      \pgfmathsetmacro{\y}{\y+1};}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newtheorem{observation}{Observation}

\newcommand{\nil}{\texttt{nil}}

\newcommand{\drawarrow}{\raisebox{2pt}{\scalebox{0.7}{\tikz{ \draw[-{Latex[length=2mm, width=2mm]},  ->,>=stealth](0,0) -- (7mm,0);} }}}

% \separatorlight{num_threads}{ind}{off1}{off2} --- draw a dashed line
% after event at index ind. off1 and off2 are left and right offsets.
\newcommand{\separatorlight}[4]{
  \draw[loosely dashed] (1.5 + 0.45 + #3, -0.4*#2 -0.2) -- (#1*1.5 + 0.45 + #4, -0.4*#2 - 0.2);
}

\newcommand{\separatordark}[4]{
  \draw[thick, dash dot] (1.5 + 0.45 + #3, -0.4*#2 -0.2) -- (#1*1.5 + 0.45 + #4, -0.4*#2 - 0.2);
  \draw[thick, dash dot] (1.5 + 0.45 + #3, -0.4*#2 -0.25) -- (#1*1.5 + 0.45 + #4, -0.4*#2 - 0.25);
}

% \demarcate{num_threads}{ind1}{ind2}{off}{text} -- draw a double headed arrow
% from event at ind1 to event at ind2, with an offset of off
% to the right of the execution, label is the text
\newcommand{\demarcate}[5]{
  \draw (#1*1.5 + 0.45 + #4, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  <->,>=stealth]  (#1*1.5 + 0.45 + #4, -0.4*#3);
  \node[fill=white] (dummy) at (#1*1.5 + 0.45 + #4, -0.2*#2 -0.2*#3) {#5};
}

==> figures/fig_motivating.tex <==
%!TEX root=../main.tex

\begin{figure}[t]
\centering
\scalebox{0.9}{
\execution{4}{
\figev{1}{$\acq(\LockColorOne{\lk_1})$}
\figev{1}{$\rel(\LockColorOne{\lk_1})$}
\figev{2}{\underline{$\acq(\LockColorTwo{\lk_2})$}}
\figev{2}{$\mathbf{\Bacq(\LockColorThree{\lk_3})}$}
\figev{2}{$\wt(z)$}
\figev{2}{$\rel(\LockColorThree{\lk_3})$}
\figev{2}{$\rel(\LockColorTwo{\lk_2})$}
\figev{4}{$\acq(\LockColorOne{\lk_1})$}
\figev{4}{\underline{$\wt(y)$}}
\figev{4}{$\rd(z)$}
}
\hspace{1cm}
\execution{4}{
	\figevoffset{10}{4}{$\rel(\LockColorOne{\lk_1})$}
	\figevoffset{10}{1}{$\acq(\LockColorThree{\lk_3})$}
	\figevoffset{10}{1}{$\wt(x)$}
	\figevoffset{10}{1}{$\rd(y)$}
	\figevoffset{10}{1}{\underline{$\rel(\LockColorThree{\lk_3})$}}
	\figevoffset{10}{3}{$\acq(\LockColorThree{\lk_3})$}
	\figevoffset{10}{3}{\underline{$\rd(x)$}}
	\figevoffset{10}{3}{$\Bacq(\LockColorTwo{\lk_2})$}
	\figevoffset{10}{3}{$\rel(\LockColorTwo{\lk_2})$}
	\figevoffset{10}{3}{$\rel(\LockColorThree{\lk_3})$}
}

%\begin{tikzpicture}[]
%	\tikzset{rectangle/.append style={draw=black}}
%	\scalebox{0.84}{
%		\def\xstep{2.2}
%		\def\ystep{0.5}
%		
%		\node[rectangle, align=center] (t1) at (-1, -7){
%			$t_2, \LockColorThree{\lk_3}, \{ \LockColorTwo{\lk_2} \}$
%		};
%		\node[rectangle, align=center] (t31) at (-1, -8.7){
%			$t_3, \LockColorTwo{\lk_2}, \{ \LockColorThree{\lk_3} \}$
%		};
%	
%		\draw[->, thick, -Latex, bend right=10] ([xshift=-3mm]t1.south) to ([xshift=-3mm]t31.north);% (t31.north);
%		\draw[->, thick, -Latex, bend right=10] (t31) to (t1);
%		
%		\node[opacity=0] at (0*\xstep, 1){};
%	}
%\end{tikzpicture}
}

% \caption{
% A  trace $\tr$ with a sync-preserving deadlock, stalling $t_2$ on $e_4$ and $t_3$ on $e_{18}$.
% Underlined events indicate the slice of $\tr$ that forms a sync-preserving lower set of $\tr$,
% and serves as a valid witness for the deadlock.
% \figlabel{motivating}
% }
\caption{
A  trace $\tr$ with a sync-preserving deadlock, stalling $t_2$ on $e_4$ and $t_3$ on $e_{18}$.
\hunkar{
Modify the example to have two deadlock patterns where one of the deadlock patterns is be realizable and the other is not, in order to demonstrate that deadlock patterns are an insufficient condition.
}
}
\figlabel{motivating}
\end{figure}

==> figures/fig_motivating3.tex <==
%!TEX root=../main.tex

\begin{figure}[t]
\centering
\scalebox{0.9}{
\execution{3}{
\figev{1}{$\acq(\LockColorOne{\lk_1})$}
\figev{1}{$\acq(\LockColorTwo{\lk_2})$}
\figev{1}{$\wt(x)$}
\figev{1}{$\rel(\LockColorTwo{\lk_2})$}
\figev{1}{$\rel(\LockColorOne{\lk_1})$}
\figev{2}{$\acq(\LockColorTwo{\lk_2})$}
\figev{2}{$\rd(x)$}

\figev{2}{$\acq(\LockColorOne{\lk_1})$}
\figev{2}{$\rel(\LockColorOne{\lk_1})$}
\figev{2}{$\rel(\LockColorTwo{\lk_2})$}

\figev{3}{$\acq(\LockColorTwo{\lk_2})$}
\figev{3}{$\acq(\LockColorOne{\lk_1})$}
%\figevoffset{13}{2}{$\rd(y)$}
\figev{3}{$\rel(\LockColorOne{\lk_1})$}
\figev{3}{$\rel(\LockColorTwo{\lk_2})$}



%\figev{3}{$\acq(\LockColorOne{\lk_1})$}
%\figev{3}{$\wt(y)$}

}
}
% \hspace{1cm}
% \execution{3}{
% %\figevoffset{11}{3}{$\rel(\LockColorOne{\lk_1})$}

% \figevoffset{11}{2}{$\acq(\LockColorThree{\lk_3})$}
% \figevoffset{11}{2}{$\acq(\LockColorFour{\lk_4})$}
% %\figevoffset{13}{2}{$\rd(y)$}
% \figevoffset{11}{2}{$\rel(\LockColorFour{\lk_4})$}
% \figevoffset{11}{2}{$\rel(\LockColorThree{\lk_3})$}

% %\figevoffset{11}{1}{$\acq(\LockColorOne{\lk_1})$}
% %\figevoffset{13}{1}{$\wt(y)$}
% %\figevoffset{13}{1}{$\rel(\LockColorOne{\lk_1})$}

% \figevoffset{11}{3}{$\acq(\LockColorFour{\lk_4})$}
% \figevoffset{11}{3}{$\acq(\LockColorThree{\lk_3})$}
% %\figevoffset{13}{3}{$\rd(y)$}
% \figevoffset{11}{3}{$\rel(\LockColorThree{\lk_3})$}
% \figevoffset{11}{3}{$\rel(\LockColorFour{\lk_4})$}

% }
% %\begin{tikzpicture}[]
% %	\tikzset{rectangle/.append style={draw=black}}
% %	\scalebox{0.84}{
% %		\def\xstep{2.2}
% %		\def\ystep{0.5}
% %		
% %		\node[rectangle, align=center] (t1) at (-1, -7){
% %			$t_2, \LockColorThree{\lk_3}, \{ \LockColorTwo{\lk_2} \}$
% %		};
% %		\node[rectangle, align=center] (t31) at (-1, -8.7){
% %			$t_3, \LockColorTwo{\lk_2}, \{ \LockColorThree{\lk_3} \}$
% %		};
% %	
% %		\draw[->, thick, -Latex, bend right=10] ([xshift=-3mm]t1.south) to ([xshift=-3mm]t31.north);% (t31.north);
% %		\draw[->, thick, -Latex, bend right=10] (t31) to (t1);
% %		
% %		\node[opacity=0] at (0*\xstep, 1){};
% %	}
% %\end{tikzpicture}
% }

% \caption{
% A  trace $\tr$ with a sync-preserving deadlock, stalling $t_2$ on $e_4$ and $t_3$ on $e_{18}$.
% Underlined events indicate the slice of $\tr$ that forms a sync-preserving lower set of $\tr$,
% and serves as a valid witness for the deadlock.
% \figlabel{motivating}
% }
\caption{
A  trace $\tr$ with a sync-preserving deadlock, stalling $t_1$ on $e_2$ and $t_3$ on $e_{12}$.
}
\figlabel{motivating}
\end{figure}

==> figures/fig_scalability.tex <==
\begin{figure}[!h]
\def\scatterscale{0.192}
\def\scatterwidth{0.23\textwidth}

\centering
\begin{subfigure}[b]{\scatterwidth}
\includegraphics[scale=\scatterscale]{figures/LinkedListDeadlockTest.pdf}
\label{subfig:sca-one-lock-clique}
\caption{LinkedList}
\end{subfigure}
\begin{subfigure}[b]{\scatterwidth}
\includegraphics[scale=\scatterscale]{figures/StackDeadlockTest.pdf}
\caption{Stack}
\label{subfig:sca-skewed}
\end{subfigure}


\caption{
Scalability experiments.
}
\label{fig:scalability}
\end{figure}

==> macros.tex <==
%!TEX root = main.tex
\makeatletter
\newcommand{\pnrelbar}{%
\linethickness{\dimen2}%
\sbox\z@{$\m@th\prec$}%
\dimen@=1.1\ht\z@
\begin{picture}(\dimen@,.4ex)
\roundcap
\put(0,.2ex){\line(1,0){\dimen@}}
\put(\dimexpr 0.5\dimen@-.2ex\relax,0){\line(1,1){.4ex}}
\end{picture}%
}

\newcommand{\precneq}{\mathrel{\vcenter{\hbox{\text{\prec@neq}}}}}
\newcommand{\prec@neq}{%
\dimen2=\f@size\dimexpr.04pt\relax
\oalign{%
\noalign{\kern\dimexpr.2ex-.5\dimen2\relax}
$\m@th\prec$\cr
\noalign{\kern-.5\dimen2}
\hidewidth\pnrelbar\hidewidth\cr
}%
}
\makeatother

\newenvironment{myparagraph}[1]{\vspace*{0.38em}\noindent{\bf #1.}}{}

\SetInd{0.3em}{0.2em}

%\newlist{compactenum}{enumerate}{3} % 3 is max-depth
%\setlist[compactenum]{label=\arabic*., nosep,leftmargin=*}
%\crefname{compactenumi}{Item}{Items}
\setlist[itemize]{nosep,leftmargin=*}
\setlist[enumerate]{label=\arabic*., nosep,leftmargin=*}

% Labels and references
\newcommand{\LowerSet}{\downarrow}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\problabel}[1]{\label{prob:#1}}
\newcommand{\probref}[1]{Problem~\ref{prob:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\itmlabel}[1]{\label{itm:#1}}
\newcommand{\itmref}[1]{\ref{itm:#1}}
\newcommand{\equlabel}[1]{\label{eq:#1}}
\newcommand{\equref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
% \newcommand{\appref}[1]{ the Appendix}
\newcommand{\algolabel}[1]{\label{algo:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{algo:#1}}
\newcommand{\linelabel}[1]{\label{line:#1}}
\newcommand{\lineref}[1]{Line~\ref{line:#1}}
\newcommand{\linerangeref}[2]{Lines~\ref{line:#1}-\ref{line:#2}}
\newcommand{\secrangeref}[2]{Sections~\ref{sec:#1}-\ref{sec:#2}}

%% Math
\newcommand{\nats}{\mathbb{N}}

\newcommand{\setofthreads}{\mathsf{Threads}}
\newcommand{\threads}[1]{\setofthreads_{#1}}
\newcommand{\locks}[1]{\mathsf{Locks}_{#1}}
\newcommand{\vars}[1]{\mathsf{Vars}_{#1}}
\newcommand{\events}[1]{\mathsf{Events}_{#1}}
\newcommand{\wevents}[1]{\mathsf{WEvents}_{#1}}
%\newcommand{\reads}[1]{\mathsf{Reads}_{#1}}
%\newcommand{\writes}[1]{\mathsf{Writes}_{#1}}
\newcommand{\Reads}[1]{\mathsf{Rds}(#1)}
\newcommand{\Writes}[1]{\mathsf{Wts}(#1)}
\newcommand{\accesses}[1]{\mathsf{Accesses}_{#1}}
\newcommand{\acquires}[1]{\mathsf{Acquires}_{#1}}
\newcommand{\releases}[1]{\mathsf{Releases}_{#1}}
\newcommand{\forks}[1]{\mathsf{Forks}_{#1}}
\newcommand{\joins}[1]{\mathsf{Joins}_{#1}}
% \renewcommand{\next}[1]{\mathsf{next}_{#1}}
\newcommand{\match}[1]{\mathsf{match}_{#1}}
\newcommand{\lheld}[1]{\mathsf{HeldLks}_{#1}}
\newcommand{\nestingdepth}[1]{\mathsf{LNDepth}_{#1}}
% \newcommand{\last}[1]{\mathsf{last}_{#1}}
\newcommand{\last}[2]{\mathsf{last}^{#1}_{#2}}
\newcommand{\RF}{\operatorname{RF}}
\newcommand{\rf}[1]{\mathsf{rf}_{#1}}
\newcommand{\Otilde}{\widetilde{O}}
% \newcommand{\SyncPDOffline}{\textsf{\tt SyncPD}\xspace}
\newcommand{\SyncPDOffline}{\textsf{\tt SPDOffline}\xspace}
% \newcommand{\SyncPDOnline}{\textsf{\tt SyncPD2}\xspace}
\newcommand{\SyncPDOnline}{\textsf{\tt SPDOnline}\xspace}
\newcommand{\SyncPDOnlineSchedule}{\textsf{\tt SyncPD2-S}\xspace}
\newcommand{\dirk}{\textsf{\tt Dirk}\xspace}
\newcommand{\seqc}{\textsf{\tt SeqCheck}\xspace}
\newcommand{\dlfuzzer}{\textsf{\tt DeadlockFuzzer}\xspace}
\newcommand{\dlfshort}{\textsf{\tt DF}\xspace}
\newcommand{\syncpdshort}{\textsf{\tt SPD}\xspace}
\newcommand{\iglshort}{\textsf{\tt IGL}\xspace}
\newcommand{\normalshort}{\textsf{\tt Normal}\xspace}
\newcommand{\syncpdshortinstr}{\textsf{\tt SPD-I}\xspace}
\newcommand{\dlfshortinstr}{\textsf{\tt DF-I}\xspace}
\newcommand{\syncpdshortinstranalysis}{\textsf{\tt SPD-I+A}\xspace}
\newcommand{\dlfshortinstranalysis}{\textsf{\tt DF-I+A}\xspace}

\newcommand{\acq}{\mathtt{acq}}
\newcommand{\rel}{\mathtt{rel}}
\newcommand{\rd}{\mathtt{r}}
\newcommand{\wt}{\mathtt{w}}
\newcommand{\fork}{\mathtt{fork}}
\newcommand{\join}{\mathtt{join}}
\newcommand{\cs}{\mathtt{cs}}

\newcommand{\Bacq}{\mathtt{\bf acq}}
\newcommand{\Brel}{\mathtt{\bf rel}}
\newcommand{\Brd}{\mathtt{\bf r}}
\newcommand{\Bwt}{\mathtt{\bf w}}
\newcommand{\Bfork}{\mathtt{\bf fork}}
\newcommand{\Bjoin}{\mathtt{\bf join}}
\newcommand{\Bcs}{\mathtt{\bf cs}}


% \newcommand{\trbegin}{\rhd}
% \newcommand{\trend}{\lhd}
% \newcommand{\trbeginfig}{\texttopcorner\textcorner}
% \newcommand{\trbeginfig}{\;\raisebox{1.3mm}{\rule{0.4pt}{1.14mm}\raisebox{1mm}{\rule{4mm}{0.4pt}}\rule{0.4pt}{1.14mm} } }
% \newcommand{\trendfig}{\;\raisebox{-0.075mm}{\rule{0.4pt}{1.14mm}\rule{4mm}{0.4pt}\rule{0.4pt}{1.14mm} } }
% \newcommand{\trbegintext}{\;\raisebox{0mm}{\rule{1pt}{1.35mm}\raisebox{1mm}{\rule{3mm}{1pt}}\rule{1pt}{1.35mm} } }
% \newcommand{\trendtext}{\;\raisebox{-0.075mm}{\rule{1pt}{1.35mm}\rule{3mm}{1pt}\rule{1pt}{1.35mm} } }
% \newcommand{\trbegin}{{\protect\trbegintext}\!}
% \newcommand{\trend}{{\protect\trendtext}\!}
\newcommand{\trbegin}{\rhd}
\newcommand{\trend}{\lhd}
\newcommand{\trbeginfig}{\rhd}
\newcommand{\trendfig}{\lhd}
\newcommand{\sync}{\mathtt{sync}}
\newcommand{\lk}{\ell}
\newcommand{\ev}[1]{\langle #1\rangle}
\newcommand{\tr}{\sigma}
\newcommand{\conf}{\asymp}
\newcommand{\comp}{\circ}
\newcommand{\wrap}{\mathtt{wrap}}
\newcommand{\clear}{\mathtt{clear}}
\newcommand{\src}{\mathtt{src}}
\newcommand{\thread}{t}
\newcommand{\ThreadOf}[1]{\operatorname{thread}(#1)}
\newcommand{\op}{\mathsf{op}}
\newcommand{\OpOf}[1]{\operatorname{op}(#1)}
\newcommand{\trnsc}{\mathsf{txn}}
\newcommand{\crit}[1]{\mathsf{CS}_{#1}}
\newcommand{\addfresh}{\mathsf{addFresh}}
\newcommand{\W}[1]{\mathsf{W[#1]}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\poly}[1]{\text{poly}(#1)}
\newcommand{\Lang}{\mathcal{L}}
\newcommand{\EQ}{\mathcal{L'}}
\newcommand{\Transducer}{\mathcal{A}}

\newcommand{\Paragraph}[1]{\smallskip\noindent{\bf #1.}}
\newcommand{\SubParagraph}[1]{\smallskip\noindent{\em #1.}}
\newcommand{\RFPoset}{\mathcal{P}}
\newcommand{\RFPosetQ}{\mathcal{Q}}
\newcommand{\RFPosetS}{\mathcal{S}}
\newcommand{\Unordered}[4]{#1\parallel^{#2}_{#3} #4}
\newcommand{\Ordered}[4]{#1 \not \parallel^{#2}_{#3} #4}
\newcommand{\Project}{|}
\newcommand{\Refines}{\sqsubseteq}
\newcommand{\SeqTrace}{\pi}
\newcommand{\ov}{\overline}
\newcommand{\ReadTriplets}[1]{\mathsf{Triplets(#1)}}
\newcommand{\DistinguishedTriplet}{\lambda}
\newcommand{\NumAcquires}{\mathcal{A}}
\newcommand{\NestingDepth}{d}
\newcommand{\NumVariables}{\mathcal{V}}
\newcommand{\NumThreads}{\mathcal{T}}
\newcommand{\NumEvents}{\mathcal{N}}
\newcommand{\NumLocks}{\mathcal{L}}

\newcommand{\NumRedEvents}{\ov{\mathcal{N}}}
\newcommand{\NumRedLocks}{\ov{\mathcal{L}}}
\newcommand{\NumRedAcquires}{\ov{\mathcal{A}}}
\newcommand{\NumRedVariables}{\ov{\mathcal{V}}}
\newcommand{\NumRedThreads}{\ov{\mathcal{T}}}


\newcommand{\set}[1]{\{#1\}}
\newcommand{\setpred}[2]{\{#1 \,|\, #2\}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\powset}[1]{\mathcal{P}(#1)}

\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
<5> <6> <7> <8> <9> <10> gen * mathb
<10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
}{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
% \DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"88}
% \DeclareMathSymbol{\varsqsubsetneq} {3}{mathb}{"8A}
% \DeclareMathSymbol{\varsqsubsetneqq}{3}{mathb}{"92}
\DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"8A}

\newcommand{\ord}[2]{\leq^{#1}_{\mathsf{#2}}}
\newcommand{\notord}[2]{{\not\leq}^{#1}_{\mathsf{#2}}}
\newcommand{\strictord}[2]{<^{#1}_{\mathsf{#2}}}
\newcommand{\trord}[1]{\leq^{#1}_{\mathsf{tr}}}
\newcommand{\stricttrord}[1]{<^{#1}_{\mathsf{tr}}}
\newcommand{\tho}[1]{\leq^{#1}_{\mathsf{TO}}}
\newcommand{\TO}{TO}
\newcommand{\stricttho}[1]{<^{#1}_{\mathsf{TO}}}
\newcommand{\nottho}[1]{\not\leq^{#1}_{\mathsf{TO}}}
% \newcommand{\stricttrord}[1]{<^{#1}_{\mathsf{tr}}}
\newcommand{\hb}[1]{\leq^{#1}_{\mathsf{HB}}}
\newcommand{\sdp}[1]{\leq^{#1}_{\mathsf{SDP}}}
\newcommand{\chb}[1]{\leq^{#1}_{\mathsf{CHB}}}
%\newcommand{\thb}[1]{<^{#1}_{\mathsf{THB}}}
\newcommand{\thb}[1]{\lessdot^{#1}_{\mathsf{Txn}}}
% \newcommand{\pth}[1]{\stackrel{*, #1}{\longrightarrow}}
\newcommand{\pth}[1]{\stackrel{*}{\longrightarrow_{#1}}}
\newcommand{\nedg}[1]{\lessdot^{#1}_{\mathsf{E}}}
\newcommand{\cp}[1]{\leq^{#1}_{\mathsf{CP}}}
\newcommand{\wcp}[1]{\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\shb}[1]{\leq^{#1}_{\mathsf{SHB}}}
\newcommand{\notwcp}[1]{\not\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\notsdp}[1]{\not\leq^{#1}_{\mathsf{SDP}}}
\newcommand{\strictwcp}[1]{\prec^{#1}_{\mathsf{WCP}}}
\newcommand{\strictshb}[1]{\strictord{#1}{\mathsf{SHB}}}
\newcommand{\ccp}[1]{\leq^{#1}_{\mathsf{DCP}}}
\newcommand{\notccp}[1]{\not\leq^{#1}_{\mathsf{DCP}}}
\newcommand{\strictccp}[1]{\prec^{#1}_{\mathsf{DCP}}}
\newcommand{\conc}[2]{\,||^{#1}_{\mathsf{#2}}\,}
\newcommand{\wcpconc}[1]{\,||^{#1}_{\mathsf{WCP}}\,}
\newcommand{\ccpconc}[1]{\,||^{#1}_{\mathsf{DCP}}\,}
\newcommand{\prev}[1]{\textsf{pred}_{#1}}
\newcommand{\trf}[1]{\leq^{#1}_{\mathsf{TRF}}}

\newcommand{\ccprank}[2]{\mathsf{rank}_\mathsf{DCP}^{#1}(#2)}
\newcommand{\wcprank}[2]{\mathsf{rank}_\mathsf{WCP}^{#1}(#2)}

\newcommand{\synctr}[1]{\mathsf{syncTrace}(#1)}
\newcommand{\unsynctr}[1]{\mathsf{unSyncTrace}(#1)}
\newcommand{\synctrev}[2]{\mathsf{syncTrace}^{#2}(#1)}
\newcommand{\freshvar}{\mathsf{fvar}}
\newcommand{\fsync}{\mathsf{first}\sync}
\newcommand{\lsync}{\mathsf{last}\sync}

\newcommand{\lw}[1]{\mathsf{lw}_{#1}}
\newcommand{\RFTrace}[1]{\lw{#1}}
\newcommand{\proj}[2]{#1|_{#2}}
\newcommand{\pattern}[1]{\tuple{#1}}
\newcommand{\sequence}[1]{[#1]}

\newcommand{\rtext}[1]{\textcolor{orange}{\sout{#1}}}
\newcommand{\atext}[1]{\textcolor{blue}{#1}}
\newcommand{\qtext}[1]{\textcolor{green}{#1}}

\def \darkred {black!20!red}
\def \darkgreen {black!40!green}

\newcommand{\LockColorOne}[1]{\textcolor{blue}{#1}}
\newcommand{\LockColorTwo}[1]{\textcolor{\darkred}{#1}}
\newcommand{\LockColorThree}[1]{\textcolor{\darkgreen}{#1}}
\newcommand{\LockColorFour}[1]{\textcolor{brown}{#1}}

\newcommand{\Andreas}[1]{\textcolor{blue}{AP:~#1}}
\newcommand{\ucomment}[1]{\textcolor{red}{#1}}
\newcommand{\hunkar}[1]{\textcolor{\darkgreen}{#1}}
\newcommand{\hcomment}[1]{\textcolor{orange}{#1}}
%\newcommand\mycommfont[1]{\ttfamily{#1}}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{gray}{#1}}
\newcommand{\cre}{\mathsf{CR}}
\SetCommentSty{mycommfont}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\renewcommand{\emptyset}{\varnothing}

%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{conjecture}{Conjecture}
% \newtheorem{observation}{Observation}

\theoremstyle{remark}
\newtheorem{remark}{Remark}

\newcommand{\closurefun}{\texttt{ComputeSPIdeal}\xspace}
\newcommand{\racefun}{\texttt{checkRace}\xspace}


\input{exec_macros}
\input{pseudocode_macros}

% \newcommand{\trzero}{\rho_1}
% \newcommand{\trone}{\rho_2}
% \newcommand{\trtwo}{\rho_3}
% \newcommand{\trthree}{\rho_4}
% \newcommand{\trfour}{\rho_8}
% \newcommand{\trfive}{\rho_9}
% \newcommand{\trsix}{\rho_6}
% \newcommand{\trseven}{\rho_7}
% \newcommand{\treight}{\rho_5}
% \newcommand{\trnine}{\rho_{10}}
% \newcommand{\trten}{\rho_{11}}

% \newcommand{\nest}[2]{\mathtt{nest}(#1\!\rightarrow\! #2)}
\newcommand{\nest}[2]{\mathtt{nest}(#1,#2)}
% \newcommand{\figevnest}[3]{\figev{#1}{ \nest{#2}{#3} } }
\newcommand{\figevnest}[3]{ \figev{#1}{\acq(#2)}\figev{#1}{\acq(#3)}\figev{#1}{\rel(#3)}\figev{#1}{\rel(#2)} }

\newcommand{\toolname}{\textsc{RAPID}\xspace}
\newcommand{\lhist}{\mathsf{History}}

\newcommand{\djitp}{\textsc{Djit}+}

% \newcommand{\vc}[1]{\!\texttt{#1}\!}
\newcommand{\vc}[1]{$\langle${\texttt{#1}}$\rangle$}


% \newcommand{\abst}[1]{\widehat{#1}}
\newcommand{\abst}[1]{{#1}^{\textsf{abs}}}
\newcommand{\SyncPAlgo}{\textsf{SyncP}\xspace}
\newcommand{\SPClosure}[1]{\mathsf{SPClosure}_{#1}}
\newcommand{\SPIdeal}[1]{\mathsf{SPIdeal}_{#1}}
\newcommand{\TOOClosure}[1]{\mathsf{TLClosure}_{#1}}

\newcommand{\lkevgraph}[1]{\mathsf{ALG}_{#1}}

%%%%%%%%%% Trace numbers %%%%%%%%%%
\newcounter{count}

\newcommand\generator[1]%
{%
  \stepcounter{count}%
  \expandafter\edef\csname#1\endcsname{\thecount}%
}

\generator{two}
\generator{one}
\generator{exampleone}
\generator{exampletwo}
\generator{examplethree}
\generator{examplefour}
\generator{three}
\generator{four}
\generator{five}
\generator{six}




==> offline-summary.tex <==
%!TEX root = main.tex
\subsection{Overall Algorithm}
\seclabel{overall-offline}





==> ov-hardness-pattern-construction.tex <==
%!TEX root = main.tex

\begin{proof}
	We show a fine-grained reduction from the Orthogonal Vectors Problem to
	the problem of checking for deadlock patterns of size $k$.
	For this, we start with two sets
	$A_1, A_2, \ldots, A_k \subseteq \set{0, 1}^d$
	of $d$-dimensional vectors with $|A_i| = n$ for every $1 \leq i \leq k$.
	We write the $j^{th}$ vector in $A_i$ as $A_{i, j}$.
	
	%\input{figures/construction-ov-hardness}
	
	\myparagraph{Construction}{
		We will construct a trace $\tr$ such that $\tr$ has a deadlock
		pattern of length $k$ iff $(A_1, A_2, \ldots, A_k)$ is a positive $k$-OV instance.
		The trace $\tr$ is of the form $\tr = \tr^{A_1} \cdot \tr^{A_2} \cdots \tr^{A_k}$
		and uses $k$ threads $\set{t_{A_1}, \ldots, t_{A_k}}$ and $d+k$ distinct 
		locks $\lk_1, \ldots, \lk_d, m_1, m_2, \ldots, m_k$. 
		Intuitively, the sub-trace $\tr^{A_i}$ encodes the given set of vectors $A_i$.
		The sub-traces $\tr^{A_i} = \tr^{A_i}_1 \cdot \tr^{A_i}_2 \cdots \tr^{A_i}_n$
		% and $\tr^B = \tr^B_1 \cdot \tr^B_2 \cdots \tr^B_n$ 
		are defined as follows.
		For each $j \in \set{1, 2, \ldots, n}$
		the sub-trace $\tr^{A_i}_j$ is the unique string generated by the
		grammar having $d+1$ non-terminals $S_0, S_1, \ldots, S_d$, start symbol $S_d$
		and the following production rules:
		\begin{itemize}
			\item $S_0 \to \ev{t_Z, \acq(m_i)} \cdot \ev{t_Z, \acq(m_{i \% k + 1})} \cdot \ev{t_Z, \rel(m_{i \% k + 1})} \cdot \ev{t_Z, \rel(m_i)}$.
			% where $(m, m') = (\lk, \lk')$ if $Z = A$, and $(m, m') = (\lk', \lk)$.
			\item for each $1 \leq p \leq d$, $S_p \to S_{p-1}$ if $A_{i, j}[p] = 0$.
			Otherwise (if $A_{i, j}[p] =1$), $S_p \to \ev{t_{A_i}, \acq(\lk_p)} \cdot S_{p-1} \cdot \ev{t_{A_i}, \rel(\lk_p)}$.
		\end{itemize}
		In words, all events of $\tr^{A_i}$ are performed by thread $t_{A_i}$.
		 % and those in $\tr^B$ are performed by $t_B$.
		Next, the $j^{th}$ sub-trace of $\tr^{A_i}$, denoted $\tr^{A_i}_j$ corresponds to the vector $A_{i, j}$
		as follows --- $\tr^{A_i}_j$ is a nested block of critical sections,
		with the innermost critical section being on lock $m_{i \% k + 1}$,
		which is immediately enclosed in a  critical section on lock $m_i$.
		Further, in the sub-trace $\tr^{A_i}_j$, 
		the lock $\lk_p$ occurs iff $A_{i, j}[p] = 1$.
		% The sub-traces $\tr^B_i$ is similarly constructed, except that the order
		% of the two innermost critical sections is inverted.
		\figref{ov-hardness} illustrates the construction for an OV-instance with $k=2$ $n=2$ and $d=2$.
	}
\end{proof}


==> ov-hardness-pattern.tex <==
%!TEX root = main.tex

\subsection{Proof of \thmref{pattern-ov-hardness}}
\seclabel{ov-hardness}




\patternovhardness*
\begin{proof}
	
	We show a fine-grained reduction from the Orthogonal Vectors Problem to
	the problem of checking for deadlock patterns of size $k$.
	For this, we start with two sets
	$A_1, A_2, \ldots, A_k \subseteq \set{0, 1}^d$
	of $d$-dimensional vectors with $|A_i| = n$ for every $1 \leq i \leq k$.
	We write the $j^{th}$ vector in $A_i$ as $A_{i, j}$.
	
	%\input{figures/construction-ov-hardness}
	
	\myparagraph{Construction}{
		We will construct a trace $\tr$ such that $\tr$ has a deadlock
		pattern of length $k$ iff $(A_1, A_2, \ldots, A_k)$ is a positive $k$-OV instance.
		The trace $\tr$ is of the form $\tr = \tr^{A_1} \cdot \tr^{A_2} \cdots \tr^{A_k}$
		and uses $k$ threads $\set{t_{A_1}, \ldots, t_{A_k}}$ and $d+k$ distinct 
		locks $\lk_1, \ldots, \lk_d, m_1, m_2, \ldots, m_k$. 
		Intuitively, the sub-trace $\tr^{A_i}$ encodes the given set of vectors $A_i$.
		The sub-traces $\tr^{A_i} = \tr^{A_i}_1 \cdot \tr^{A_i}_2 \cdots \tr^{A_i}_n$
		% and $\tr^B = \tr^B_1 \cdot \tr^B_2 \cdots \tr^B_n$ 
		are defined as follows.
		For each $j \in \set{1, 2, \ldots, n}$
		the sub-trace $\tr^{A_i}_j$ is the unique string generated by the
		grammar having $d+1$ non-terminals $S_0, S_1, \ldots, S_d$, start symbol $S_d$
		and the following production rules:
		\begin{itemize}
			\item $S_0 \to \ev{t_Z, \acq(m_i)} \cdot \ev{t_Z, \acq(m_{i \% k + 1})} \cdot \ev{t_Z, \rel(m_{i \% k + 1})} \cdot \ev{t_Z, \rel(m_i)}$.
			% where $(m, m') = (\lk, \lk')$ if $Z = A$, and $(m, m') = (\lk', \lk)$.
			\item for each $1 \leq p \leq d$, $S_p \to S_{p-1}$ if $A_{i, j}[p] = 0$.
			Otherwise (if $A_{i, j}[p] =1$), $S_p \to \ev{t_{A_i}, \acq(\lk_p)} \cdot S_{p-1} \cdot \ev{t_{A_i}, \rel(\lk_p)}$.
		\end{itemize}
		In words, all events of $\tr^{A_i}$ are performed by thread $t_{A_i}$.
		 % and those in $\tr^B$ are performed by $t_B$.
		Next, the $j^{th}$ sub-trace of $\tr^{A_i}$, denoted $\tr^{A_i}_j$ corresponds to the vector $A_{i, j}$
		as follows --- $\tr^{A_i}_j$ is a nested block of critical sections,
		with the innermost critical section being on lock $m_{i \% k + 1}$,
		which is immediately enclosed in a  critical section on lock $m_i$.
		Further, in the sub-trace $\tr^{A_i}_j$, 
		the lock $\lk_p$ occurs iff $A_{i, j}[p] = 1$.
		% The sub-traces $\tr^B_i$ is similarly constructed, except that the order
		% of the two innermost critical sections is inverted.
		\figref{ov-hardness} illustrates the construction for an OV-instance with $k=2$ $n=2$ and $d=2$.
	}

\myparagraph{Correctness}{
We now argue for the correctness of the construction.
First, if $(A_1, A_2, \ldots, A_k)$ is a positive $OV$ instance, then
there are $k$ indices $\alpha_1, \alpha_2, \ldots, \alpha_k \in \set{1 ,\ldots, n}$
such that $\sum_{p=1}^d \prod_{i=1}^k A_{i, \alpha_i}[p] = 0$.
 % and $B_\beta$ are orthogonal.
Thus, for every $1 \leq p \leq d$, there is an $i$ such that $A_{i, \alpha_i}[p] = 0$.
% or $B_\beta[j] = 0$.
Based on the construction, this implies that for every lock $\lk_p$
(with $1 \leq p \leq d$),
$\lk_p$ occurs in at most one of the sub-traces $\tr^{A_1}_{\alpha_1}, \ldots, \tr^{A_k}_{\alpha_k}$.
 % and $\tr^B_\beta$.
This gives a deadlock pattern $D = \pattern{e_1, e_2, \ldots, e_k}$,
where $e_i$ is the unique event in the sub-trace $\tr^{A_i}_{\alpha_i}$ with $\OpOf{e} = \acq(m_{i\%k +1})$.
% and $e'$ is the unique event in $\tr^B_\beta$ with $\OpOf{e'} = \acq(\lk)$.
This is because $m_i \in \lheld{\tr}(e_i)$,
and each lock $\lk_p$ exists in at most one of $\set{\lheld{\tr}(e_i)}_{i\leq n}$
% or $\lheld{\tr}(e')$ 
(and thus $\lheld{\tr}(e_i) \cap \lheld{\tr}(e_{i'}) = \emptyset$ for every $i \neq i' \leq n$).

Now, consider the case when there is a deadlock pattern $D = \pattern{e_1, e_2, \ldots, e_k}$ in $\tr$.
W.l.o.g, we can assume that
$\ThreadOf{e_i} = t_{A_i}$.
This means there are $\alpha_1, \alpha_2, \ldots, \alpha_k$
 % and $\beta$ such that
 such that
$e_i$ occurs in $\tr^{A_i}_{\alpha_i}$.
 % and $e'$ occurs in $\tr^B_\beta$.
Next, observe that the events $\set{e_i}_{i \leq k}$
 % and $e'$ 
 can only be acquire events on locks $\set{m_1, m_2, \ldots, m_k}$
and not on the locks $\set{\lk_1, \ldots, \lk_d}$.
This is because the order of acquisition amongst $\lk_1, \ldots, \lk_d$
is always fixed and further, each of these are never acquired inside of critical sections
of $m_1, \ldots, m_k$.
 % or $\lk'$.
By the choice of threads, $\OpOf{e_i} = \acq(m_{i\%k + 1})$ for every $i \leq k$.
% and $\OpOf{e'} = \acq(\lk)$.
Since $\lheld{\tr}(e_i) \cap \lheld{\tr}(e_{i'}) = \emptyset$ for every $i \neq i' \leq k$, 
we also have that
for every $p \leq d$, $\lk_p \not\in \lheld{\tr}(e) \cap \lheld{\tr}(e')$.
This means that at, for each $p \leq d$, there is atmost one $i \leq k$
for which $A_{i, \alpha_i}[p] = 1$.
This means that the vectors $A_{1, \alpha_1}, A_{2, \alpha_2} \ldots, A_{k, \alpha_k}$
witness that the given OV instance is a positive instance.
}


	\myparagraph{Time complexity}{
		For any fixed $k\geq 2$, the total size of the trace is $\NumEvents = O(n\cdot d)$
		and it has $\NumLocks = d + k $ locks.
		The construction can be performed in time $O(n\cdot d)$.
		Thus, if for some $\epsilon > 0$, 
		there is a $O(\poly{\NumLocks} \cdot \NumEvents^{k-\epsilon}) = O(\poly{d} \cdot n^{k-\epsilon})$ 
		algorithm for the problem of detecting deadlock patterns of length $k$,
		we would get a $O(\poly{d} \cdot n^{k-\epsilon} + n\cdot d) = O(\poly{d} \cdot n^{k-\epsilon})$
		time algorithm for $k$-OV, falsifying the $k$-OV hypothesis.
	}
\end{proof}


==> pseudocode_macros.tex <==
%!TEX root = main.tex

%%%%%% Macros for algo %%%%%%%%
\SetKwProg{myfun}{function}{}{}
\SetKwProg{myhandler}{handler}{}{}
\SetKwFunction{init}{Initialization}
% \SetKwFunction{fixpoint}{ComputeLCClosure}
\SetKwFunction{fixpoint}{CompSPClosure}
\SetKwFunction{maxLB}{maxLowerBound}
\SetKwFunction{checkAbsDeadP}{CheckAbsDdlck}
\SetKwFunction{checkDeadlock}{checkDeadlock}
\SetKwFunction{rdhandler}{read}
\SetKwFunction{wthandler}{write}
\SetKwFunction{acqhandler}{acquire}
\SetKwFunction{relhandler}{release}
\SetKwInput{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{Let}{let}
\SetKw{Break}{break}
\SetKw{NOT}{not}
\SetKw{declare}{declare}
\SetKw{report}{report}
\SetKw{exit}{exit}
\SetKwFor{Foreach}{for each}{}{}%
\DontPrintSemicolon
% \newcommand{\ideal}{\mathsf{I}}

\newcommand{\AcqLst}{\mathsf{CSHist}}
\newcommand{\DPLst}{\mathsf{AcqHist}}

\newcommand{\mx}{\sqcup}
\newcommand{\cle}{\sqsubseteq}
\newcommand{\Cc}{\mathbb{C}}
\newcommand{\LW}{\mathbb{LW}}
\newcommand{\Ii}{\mathbb{I}}
%\newcommand{\gId}{\mathbbm{g}}
\newcommand{\gId}{{g}}
\newcommand{\lastGID}{\gId\mathsf{\_max}}
\newcommand{\lastRelTime}{\mathsf{RelTime\_max}}

\newcommand{\view}[3]{{#1}_{#2}^{#3}}

\renewcommand{\nil}{\mathtt{NIL}}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother
\newcommand{\apicall}[3]{{#1}\bigcdot{\textup{\texttt{#2(#3)}}}}
\newcommand{\first}[1]{\apicall{#1}{first}{}}
\newcommand{\removeFirst}[1]{\apicall{#1}{removeFirst}{}}
\newcommand{\isEmpty}[1]{\apicall{#1}{isEmpty}{}}
\newcommand{\lst}[1]{\apicall{#1}{last}{}}
\newcommand{\addLst}[2]{\apicall{#1}{addLast}{#2}}
\newcommand{\updateRel}[2]{\apicall{#1}{updateRelease}{#2}}

\newcommand{\true}{\top\!\!\!\!\top}
\newcommand{\false}{\bot\!\!\!\!\bot}

==> tables/dirk_results.tex <==
%!TEX root = ../main.tex

\begin{table*}[H]
\caption{
Trace characteristics, Lock graph statistics and performance comparison.
Column 1 denotes the name of the benchmark.
Columns 2, 3, 4, 5 and 6 respectively denote the number of events, threads, memory locations, locks
and the total number of acquire and request events.
Columns 7, 8 and 9 denote the number of nodes, edges and cycles in the abstract lock graph,
while Columns 10 and 11 denote the number of abstract and concrete deadlock patterns.
Columns 12 - 17 denote the times taken (in seconds) and the number of deadlocks reported
by each of Dirk, \SyncPDOnline and \SyncPDOffline.
%Statistics on the lock graph $\lkevgraph{\tr}$ of each trace $\tr$.
% We denote by $\mathcal{N}$, $\mathcal{T}$, $\mathcal{M}$, $\mathcal{L}$ and $\NumAcquires + \mathcal{R}$ the total number of events, number of threads, number of memory locations, number of locks and number of acquire and request events in the benchmarks, respectively. 
\label{tab:expr-results-dirk}
}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{0.95}
\small
\centering
\scalebox{0.96}{
\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c||c|c||c|c||c|c|}
\hline
1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 \\
\hline
\multirow{2}{*}{\textbf{Benchmark}}& 
\multirow{2}{*}{$\mathcal{N}$} & \multirow{2}{*}{$\mathcal{T}$} & \multirow{2}{*}{$\mathcal{M}$} & \multirow{2}{*}{$\mathcal{L}$} & \multirow{2}{*}{$\NumAcquires+\mathcal{R}$} 
& \multicolumn{5}{c||}{ \textsf{Abstract Lock Graph } $\lkevgraph{\tr}$}
& \multicolumn{2}{c||}{ {\textsf{Dirk}} } 
& \multicolumn{2}{c||}{ {\textsf{$\SyncPDOffline$}}} 
& \multicolumn{2}{c|}{ {\textsf{$\SyncPDOnline$}}} \\
\cline{7-17}
& & & & & 
& \textsf{|$V_\tr$|}
& \textsf{|$E_\tr$|}
& \textsf{|$\textsf{Cyc}_\tr$|}
& \textsf{\textsf{Abs. Pat.}}
& \textsf{\textsf{Conc. Pat.}}
& \textbf{\#Dlk} 
& {\textbf{Time (s)}} 
&{\textbf{\#Dlk}} 
& {\textbf{Time (s)}}
&{\textbf{\#Dlk}} 
&{\textbf{Time (s)}} \\
\hline
Deadlock & 50 & 3 & 4 & 3 & 4 & 2 & 2 & 1 & 1 & 1 & 1 & 0.02 & 0 & 0.06 & 0 & 0.03 
\\
NotADeadlock & 74 & 3 & 3 & 4 & 10 & 2 & 2 & 1 & 1 & 1 & 0 & 0.02 & 0 & 0.06 & 0 & 0.03 
\\
Picklock & 80 & 3 & 5 & 5 & 12 & 6 & 8 & 2 & 2 & 2 & 1 & 0.02 & 1 & 0.06 & 1 & 0.02 
\\
Bensalem & 86 & 4 & 4 & 4 & 12 & 6 & 6 & 2 & 2 & 2 & 1 & 0.03 & 1 & 0.06 & 1 & 0.03 
\\
Transfer & 93 & 3 & 10 & 3 & 8 & 2 & 2 & 1 & 1 & 1 & 1 & 0.03 & 0 & 0.06 & 0 & 0.03 
\\
Test & 95 & 3 & 8 & 6 & 14 & 7 & 7 & 2 & 2 & 2 & 2 & 0.06 & 2 & 0.06 & 2 & 0.03 
\\
StringBuffer & 116 & 3 & 14 & 4 & 6 & 2 & 2 & 1 & 1 & 2 & 2 & 0.03 & 2 & 0.06 & 2 & 0.03 
\\
DiningPhil & 398 & 6 & 21 & 6 & 50 & 5 & 5 & 1 & 1 & 3.1K & 1 & 2.0 & 1 & 0.07 & 0 & 0.03 
\\
HashTable & 522 & 3 & 5 & 3 & 65 & 2 & 0 & 0 & 0 & 0 & 2 & 0.23 & 2 & 0.08 & 2 & 0.03 
\\
DirkAccount & 897 & 6 & 46 & 6 & 72 & 8 & 12 & 3 & 3 & 12 & 0 & 0.27 & 0 & 0.08 & 0 & 0.03 
\\
Log4j2 & 2.5K & 4 & 334 & 11 & 15 & 1 & 0 & 0 & 0 & 0 & 1 & 0.78 & 1 & 0.07 & 1 & 0.03 
\\
Derby2 & 3.0K & 3 & 1.0K & 4 & 2 & 1 & 0 & 0 & 0 & 0 & 1 & 0.33 & 1 & 0.08 & 1 & 0.04 
\\
JDBCMySQL-1 & 674.5K & 3 & 73.1K & 11 & 4.1K & 15 & 10 & 1 & 1 & 4 & 2 & 34.5 & 2 & 0.33 & 2 & 0.26 
\\
JDBCMySQL-2 & 674.7K & 3 & 73.2K & 11 & 1.3K & 11 & 2 & 0 & 0 & 0 & 1 & 37.1 & 1 & 0.24 & 1 & 0.29 
\\
JDBCMySQL-3 & 675.9K & 3 & 73.2K & 12 & 4.1K & 22 & 23 & 5 & 5 & 16 & 1 & 115.6 & 1 & 0.34 & 1 & 0.33 
\\
JDBCMySQL-4 & 676.0K & 3 & 73.3K & 13 & 4.1K & 21 & 21 & 5 & 4 & 18 & 2 & 189.2 & 2 & 0.51 & 2 & 0.34 
\\
ArrayList & 4.1M & 801 & 120.6K & 802 & 81.4K & 115 & 8 & 4 & 4 & 301 & - & - & 3 & 1.9 & 3 & 1.6 
\\
Stack & 4.4M & 801 & 118.3K & 1.6K & 165.9K & 1.9K & 246 & 3 & 3 & 201 & - & - & 3 & 4.2 & 3 & 3.1 
\\
IdentityHashMap & 4.5M & 801 & 496.1K & 802 & 80.9K & 40 & 2 & 1 & 1 & 4 & - & - & 1 & 1.7 & 1 & 1.7 
\\
LinkedList & 4.8M & 801 & 289.9K & 802 & 81.3K & 114 & 8 & 4 & 4 & 10.2K & - & - & 3 & 2.5 & 3 & 2.1 
\\
HashMap & 5.3M & 801 & 554.7K & 802 & 84.6K & 40 & 2 & 1 & 1 & 10.2K & - & - & 2 & 2.0 & 2 & 2.0 
\\
Vector & 5.4M & 3 & 14 & 3 & 400.0K & 2 & 2 & 1 & 1 & 1.4B & - & - & 1 & 2.2 & 1 & 1.2 
\\
LinkedHashMap & 6.2M & 801 & 617.0K & 802 & 84.6K & 40 & 2 & 1 & 1 & 10.2K & - & - & 2 & 1.9 & 2 & 2.3 
\\
WeakHashMap & 6.3M & 801 & 540.4K & 802 & 84.5K & 40 & 2 & 1 & 1 & 10.2K & - & - & 2 & 1.9 & 2 & 2.1 
\\
TreeMap & 19.5M & 801 & 493.4K & 802 & 84.6K & 40 & 2 & 1 & 1 & 10.2K & - & - & 2 & 3.0 & 2 & 2.5 
\\
TestPerf & 200.1M & 50 & 599 & 9 & 98.3K & 0 & 0 & 0 & 0 & 0 & - & - & 0 & 16.0 & 0 & 7.9 
\\
Groovy2 & 212.8M & 13 & 12.7M & 9.9K & 10.8K & 13 & 0 & 0 & 0 & 0 & - & - & 0 & 15.5 & 0 & 13.3 
\\
\hline
\hline
\textbf{Total} & \textbf{476M} & & \textbf{16M} & \textbf{17k} & \textbf{1.2M} 
& \textbf{2.4K} & \textbf{376} & \textbf{42} & \textbf{41} & \textbf{1.4B}
& \textbf{19} & \textbf{>380} & \textbf{36} & \textbf{55} & \textbf{35} & \textbf{41}
\\
\hline
\end{tabular}
}
\end{table*}


==> tables/dirk_results_old.tex <==
%!TEX root = ../main.tex

\begin{table*}[b]
\caption{
We denote by $\mathcal{N}$, $\mathcal{T}$, $\mathcal{M}$, $\mathcal{L}$ and $\mathcal{R}$ the total number of events, number of threads, number of memory locations, number of locks and number of request events in the benchmarks, respectively. 
\label{tab:expr-results-dirk-2}
}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{0.95}
\small
\centering
\begin{tabular}{|c|c|c|c|c|c||c|c||c|c||c|c|}
\hline
\multirow{2}{*}{\textbf{Benchmark}}& \multirow{2}{*}{$\mathcal{N}$} & \multirow{2}{*}{$\mathcal{T}$} & \multirow{2}{*}{$\mathcal{M}$}
& \multirow{2}{*}{$\mathcal{L}$} &
\multirow{2}{*}{$\mathcal{R}$} &\multicolumn{2}{c||}{ {\textsf{Dirk}}} & \multicolumn{2}{c||}{ {\textsf{$\SyncPDOnline$}}} & \multicolumn{2}{c|}{ {\textsf{$\SyncPDOffline$}}} \\
\cline{7-12}
& & & & & &  \textbf{$\#$Deadlocks} & { \textbf{Time (s)}} &{ \textbf{$\#$Deadlocks}} & { \textbf{Time (s)}} &{ \textbf{$\#$Deadlocks}} &{ \textbf{Time (s)}} \\
\hline
Deadlock & 50 & 3 & 4 & 3 & 4 & 1 & 0.024 & 0 & 0.024 & 0 & 0.063
\\
NotADeadlock & 74 & 3 & 3 & 4 & 6 & 0 & 0.020 & 0 & 0.029 & 0 & 0.064
\\
Picklock & 80 & 3 & 5 & 5 & 8 & 1 & 0.028 & 1 & 0.025 & 1 & 0.058
\\
Bensalem & 86 & 4 & 4 & 4 & 10 & 1 & 0.032 & 1 & 0.025 & 1 & 0.064
\\
Transfer & 93 & 3 & 10 & 3 & 4 & 1 & 0.034 & 0 & 0.025 & 0 & 0.057
\\
Test & 95 & 3 & 8 & 6 & 10 & 2 & 0.064 & 2 & 0.026 & 2 & 0.064
\\
StringBuffer & 116 & 3 & 14 & 4 & 8 & 2 & 0.034 & 2 & 0.025 & 2 & 0.062
\\
DiningPhil & 398 & 6 & 21 & 6 & 50 & 1 & 2.010 & 0 & 0.029 & 1 & 0.074
\\
HashTable & 522 & 3 & 5 & 3 & 67 & 2 & 0.233 & 2 & 0.031 & 2 & 0.078
\\
DirkAccount & 897 & 6 & 46 & 6 & 62 & 0 & 0.272 & 0 & 0.029 & 0 & 0.080
\\
Log4j2 & 2.4K & 4 & 334 & 11 & 18 & 1 & 0.781 & 1 & 0.032 & 1 & 0.066
\\
Derby2 & 3.0K & 3 & 1.0K & 4 & 4 & 1 & 0.327 & 1 & 0.035 & 1 & 0.080
\\
JDBCMySQL-1 & 674.5K & 3 & 73.1K & 11 & 4.0K & 2 & 34.554 & 2 & 0.339 & 2 & 0.327
\\
JDBCMySQL-2 & 674.6K & 3 & 73.1K & 11 & 1.2K & 1 & 37.099 & 1 & 0.336 & 1 & 0.241
\\
JDBCMySQL-3 & 675.8K & 3 & 73.2K & 12 & 4.0K & 1 & 115.634 & 1 & 0.347 & 1 & 0.343
\\
JDBCMySQL-4 & 675.9K & 3 & 73.2K & 13 & 4.0K & 2 & 189.190 & 2 & 0.422 & 2 & 0.511
\\
Vector & 5.4M & 3 & 14 & 3 & 400.0K & - & T.O. & 1 & 1.483 & 1 & 2.172
\\
TestPerf & 200.0M & 50 & 599 & 9 & 98.2K & - & T.O. & 0 & 9.494 & 0 & 16.026
\\
Groovy2 & 212.7M & 13 & 12.7M & 9.8K & 10.8K & - & T.O. & 0 & 14.960 & 0 & 15.480
\\
\hline
\hline
\textbf{Total} & \textbf{1.5B} & & \textbf{68.0M} & \textbf{29.8K} & \textbf{998.6K} & \textbf{19} & \textbf{>538.151} & \textbf{17} & \textbf{14.919} & \textbf{18} & \textbf{22.791}
\\
\hline
\end{tabular}
\end{table*}


==> tables/tab_cycles.tex <==
%!TEX root = ../main.tex

\begin{table}
\caption{
Statistics on the lock graph $\lkevgraph{\tr}$ of each trace $\tr$.
}
\label{tab:expr-cycles}
\setlength\tabcolsep{2pt}
\renewcommand{\arraystretch}{0.93}
\small
\centering
\scalebox{0.96}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{
\textbf{Benchmark}} &
 \multirow{3}{*}{\textbf{Nodes}} & \multirow{3}{*}{\textbf{Edges}} & \multirow{3}{*}{\textbf{Cycles}} & 
\multirowcell{3}{\textbf{Abstract} \\ \textbf{Deadlock} \\
\textbf{Patterns}} &
\multirowcell{3}{\textbf{Concrete} \\ \textbf{Deadlock} \\ \textbf{Patterns}}
\\ & & & & &\\ & & & & & \\
\hline
Deadlock & 2 & 2 & 1 & 1 & 1\\
NotADeadlock & 2 & 2 & 1 & 1 & 1\\
Picklock & 6 & 8 & 2 & 2 & 2\\
Bensalem & 6 & 6 & 2 & 2 & 2\\
Transfer & 2 & 2 & 1 & 1 & 1\\
Test & 7 & 7 & 2 & 2 & 2\\
StringBuffer & 2 & 2 & 1 & 1 & 2\\
DiningPhil & 5 & 5 & 1 & 1 & 3.12K\\
HashTable & 2 & 0 & 0 & 0 & 0\\
DirkAccount & 8 & 12 & 3 & 3 & 12\\
Log4j2 & 1 & 0 & 0 & 0 & 0\\
Dbcp1 & 9 & 6 & 2 & 2 & 3\\
Derby2 & 1 & 0 & 0 & 0 & 0\\
Dbcp2 & 6 & 4 & 1 & 1 & 4\\
JDBCMySQL-1 & 15 & 10 & 1 & 1 & 4\\
JDBCMySQL-2 & 11 & 2 & 0 & 0 & 0\\
JDBCMySQL-3 & 22 & 23 & 5 & 5 & 16\\
JDBCMySQL-4 & 21 & 21 & 5 & 4 & 18\\
jigsaw-1 & 89 & 101 & 1 & 1 & 8\\
jigsaw-2 & 180 & 324 & 7 & 6 & 83\\
ArrayList & 115 & 8 & 4 & 4 & 301\\
Stack & 1.88K & 246 & 3 & 3 & 201\\
IdentityHashMap & 40 & 2 & 1 & 1 & 4\\
LinkedList & 114 & 8 & 4 & 4 & 10.20K\\
HashMap & 40 & 2 & 1 & 1 & 10.20K\\
Vector & 2 & 2 & 1 & 1 & 1.41B\\
LinkedHashMap & 40 & 2 & 1 & 1 & 10.20K\\
WeakHashMap & 40 & 2 & 1 & 1 & 10.20K\\
montecarlo & 0 & 0 & 0 & 0 & 0\\
TreeMap & 40 & 2 & 1 & 1 & 10.20K\\
hsqldb & 505 & 28.60K & 0 & 0 & 0\\
sunflow & 16 & 0 & 0 & 0 & 0\\
TestPerf-1 & 0 & 0 & 0 & 0 & 0\\
tradesoap & 1.55K & 4.46K & 2 & 2 & 4\\
tradebeans & 1.56K & 4.46K & 2 & 2 & 4\\
jspider & 49 & 40 & 0 & 0 & 0\\
eclipse & 6.67K & 81.82K & 9 & 7 & 280\\
TestPerf-2 & 0 & 0 & 0 & 0 & 0\\
Groovy2 & 13 & 0 & 0 & 0 & 0\\
biojava & 25 & 1 & 0 & 0 & 0\\
graphchi & 11 & 0 & 0 & 0 & 0\\
batik & 0 & 0 & 0 & 0 & 0\\
\hline
\end{tabular}
}
\end{table}


==> tables/tab_experiments.tex <==
%!TEX root = ../main.tex

\begin{table*}
\caption{
We denote by $\mathcal{N}$, $\mathcal{T}$, $\mathcal{M}$, $\mathcal{L}$ and $\NumAcquires + \mathcal{R}$ the total number of events, number of threads, number of memory locations, number of locks and number of acquire and request events in the benchmarks, respectively. 
\label{tab:expr-results}
}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{0.95}
\small
\centering
\scalebox{0.96}{
\begin{tabular}{|c|c|c|c|c|c||c|c||c|c||c|c|}
\hline
\multirow{2}{*}{\textbf{Benchmark}}& \multirow{2}{*}{$\mathcal{N}$} & \multirow{2}{*}{$\mathcal{T}$} & \multirow{2}{*}{$\mathcal{M}$}
& \multirow{2}{*}{$\mathcal{L}$} &
\multirow{2}{*}{$\NumAcquires+\mathcal{R}$} &\multicolumn{2}{c||}{ {\seqc}} & \multicolumn{2}{c||}{ {\textsf{$\SyncPDOffline$}}} & \multicolumn{2}{c|}{ {\textsf{$\SyncPDOnline$}}} \\
\cline{7-12}
& & & & & &  \textbf{$\#$Deadlocks} & { \textbf{Time (s)}} &{ \textbf{$\#$Deadlocks}} & { \textbf{Time (s)}} &{ \textbf{$\#$Deadlocks}} &{ \textbf{Time (s)}} \\
\hline
Deadlock & 50 & 3 & 4 & 3 & 4 & 0 & 0.051 & 0 & 0.063 & 0 & 0.026
\\
NotADeadlock & 74 & 3 & 3 & 4 & 10 & 0 & 0.052 & 0 & 0.064 & 0 & 0.028
\\
Picklock & 80 & 3 & 5 & 5 & 12 & 1 & 0.059 & 1 & 0.058 & 1 & 0.024
\\
Bensalem & 86 & 4 & 4 & 4 & 12 & 1 & 0.058 & 1 & 0.064 & 1 & 0.034
\\
Transfer & 93 & 3 & 10 & 3 & 8 & 0 & 0.048 & 0 & 0.057 & 0 & 0.03
\\
Test & 95 & 3 & 8 & 6 & 14 & 2 & 0.051 & 2 & 0.064 & 2 & 0.026
\\
StringBuffer & 116 & 3 & 14 & 4 & 6 & 2 & 0.053 & 2 & 0.062 & 2 & 0.025
\\
DiningPhil & 398 & 6 & 21 & 6 & 50 & 0 & 0.05 & 1 & 0.074 & 0 & 0.027
\\
HashTable & 522 & 3 & 5 & 3 & 65 & 2 & 0.074 & 2 & 0.078 & 2 & 0.03
\\
DirkAccount & 897 & 6 & 46 & 6 & 72 & 0 & 0.053 & 0 & 0.08 & 0 & 0.027
\\
Log4j2 & 2.47K & 4 & 334 & 11 & 15 & 1 & 0.057 & 1 & 0.066 & 1 & 0.03
\\
Dbcp1 & 2.90K & 3 & 768 & 5 & 14 & 2 & 0.06 & 2 & 0.068 & 2 & 0.031
\\
Derby2 & 3.03K & 3 & 1.01K & 4 & 2 & 1 & 0.077 & 1 & 0.08 & 1 & 0.041
\\
Dbcp2 & 4.09K & 3 & 592 & 10 & 22 & 0 & 0.057 & 0 & 0.083 & 0 & 0.044
\\
JDBCMySQL-1 & 674.54K & 3 & 73.14K & 11 & 4.08K & 2 & 0.273 & 2 & 0.327 & 2 & 0.262
\\
JDBCMySQL-2 & 674.69K & 3 & 73.19K & 11 & 1.28K & 1 & 0.23 & 1 & 0.241 & 1 & 0.289
\\
JDBCMySQL-3 & 675.86K & 3 & 73.25K & 12 & 4.09K & 1 & 0.25 & 1 & 0.343 & 1 & 0.328
\\
JDBCMySQL-4 & 675.99K & 3 & 73.27K & 13 & 4.10K & 2 & 0.308 & 2 & 0.511 & 2 & 0.335
\\
jigsaw-1 & 2.81M & 14 & 63.27K & 105 & 258 & 0 & 0.401 & 0 & 0.612 & 0 & 0.301
\\
jigsaw-2 & 3.20M & 15 & 103.52K & 276 & 1.07K & 0 & 1.628 & 0 & 0.744 & 0 & 0.484
\\
ArrayList & 4.06M & 801 & 120.56K & 802 & 81.42K & 3 & 22.116 & 3 & 1.851 & 3 & 1.609
\\
Stack & 4.43M & 801 & 118.27K & 1.60K & 165.90K & 3 & 20.459 & 3 & 4.189 & 3 & 3.097
\\
IdentityHashMap & 4.55M & 801 & 496.05K & 802 & 80.88K & 1 & 10.123 & 1 & 1.717 & 1 & 1.74
\\
LinkedList & 4.85M & 801 & 289.94K & 802 & 81.35K & 3 & 45.879 & 3 & 2.461 & 3 & 2.051
\\
HashMap & 5.35M & 801 & 554.70K & 802 & 84.64K & 2 & 683.553 & 2 & 1.986 & 2 & 2.036
\\
Vector & 5.40M & 3 & 14 & 3 & 400.00K & 1 & 1.787 & 1 & 2.172 & 1 & 1.17
\\
LinkedHashMap & 6.17M & 801 & 617.02K & 802 & 84.64K & 2 & 556.54 & 2 & 1.893 & 2 & 2.283
\\
WeakHashMap & 6.32M & 801 & 540.35K & 802 & 84.54K & 2 & 695.652 & 2 & 1.864 & 2 & 2.095
\\
montecarlo & 10.13M & 3 & 850.16K & 2 & 4 & 0 & 2.336 & 0 & 0.873 & 0 & 0.786
\\
TreeMap & 19.48M & 801 & 493.45K & 802 & 84.64K & 2 & 655.245 & 2 & 2.965 & 2 & 2.47
\\
hsqldb & 20.00M & 46 & 945.04K & 402 & 167.44K & 0 & - & 0 & 2.482 & 0 & 5.005
\\
sunflow & 34.85M & 16 & 2.03M & 11 & 602 & 0 & 11.095 & 0 & 2.351 & 0 & 2.459
\\
TestPerf-1 & 36.45M & 52 & 623 & 9 & 22.77K & 0 & 11.836 & 0 & 2.361 & 0 & 1.673
\\
tradesoap & 42.03M & 236 & 2.84M & 6.11K & 58.27K & 0 & 92.916 & 0 & 8.317 & 0 & 5.766
\\
tradebeans & 42.04M & 236 & 2.83M & 6.11K & 58.34K & 0 & 92.409 & 0 & 8.3 & 0 & 5.576
\\
jspider & 47.53M & 11 & 4.79M & 15 & 5.23K & 0 & 10.637 & 0 & 3.786 & 0 & 3.615
\\
eclipse & 126.28M & 15 & 10.45M & 4.69K & 161.18K & 0 & 32.867 & 0 & 15.687 & 0 & 10.255
\\
TestPerf-2 & 200.10M & 50 & 599 & 9 & 98.27K & 0 & 54.806 & 0 & 16.026 & 0 & 7.853
\\
Groovy2 & 212.76M & 13 & 12.73M & 9.89K & 10.82K & 0 & 49.639 & 0 & 15.48 & 0 & 13.266
\\
biojava & 221.13M & 6 & 121.02K & 79 & 383 & 0 & 69.125 & 0 & 12.338 & 0 & 13.392
\\
graphchi & 240.66M & 20 & 24.88M & 61 & 344 & 0 & 118.925 & 0 & 21.14 & 0 & 24.955
\\
batik & 279.91M & 7 & 5.11M & 1.92K & 56 & 0 & 17.491 & 0 & 18.094 & 0 & 15.417
\\
\hline
\hline
\textbf{Total} & \textbf{1.58B} & & \textbf{71.27M} & \textbf{37.02K} & \textbf{1.75M} & \textbf{37} & \textbf{3259.326} & \textbf{38} & \textbf{152.072} & \textbf{37} & \textbf{130.991}
\\
\hline
\end{tabular}
}
\end{table*}


==> tables/tab_merged.tex <==
%!TEX root = ../main.tex

\begin{table*}
\caption{
We denote by $\mathcal{N}$, $\mathcal{T}$, $\mathcal{M}$, $\mathcal{L}$ and $\NumAcquires + \mathcal{R}$ the total number of events, number of threads, number of memory locations, number of locks and number of acquire and request events in the benchmarks, respectively. 
\label{tab:expr-results}
}
\setlength\tabcolsep{3pt}
\renewcommand{\arraystretch}{0.95}
\small
\centering
\scalebox{0.96}{
\begin{tabular}{|c|c|c|c|c|c||c|c||c|c||c|c|}
\hline
\multirow{2}{*}{\textbf{Benchmark}}& \multirow{2}{*}{$\mathcal{N}$} & \multirow{2}{*}{$\mathcal{T}$} & \multirow{2}{*}{$\mathcal{M}$}
& \multirow{2}{*}{$\mathcal{L}$} &
\multirow{2}{*}{$\NumAcquires+\mathcal{R}$} &\multicolumn{2}{c||}{ {\seqc}} & \multicolumn{2}{c||}{ {\textsf{$\SyncPDOffline$}}} & \multicolumn{2}{c|}{ {\textsf{$\SyncPDOnline$}}} \\
\cline{7-12}
& & & & & &  \textbf{$\#$Deadlocks} & { \textbf{Time (s)}} &{ \textbf{$\#$Deadlocks}} & { \textbf{Time (s)}} &{ \textbf{$\#$Deadlocks}} &{ \textbf{Time (s)}} \\
\hline
Deadlock & 50 & 3 & 4 & 3 & 4 & 0 & 0.051 & 0 & 0.063 & 0 & 0.026
\\
NotADeadlock & 74 & 3 & 3 & 4 & 10 & 0 & 0.052 & 0 & 0.064 & 0 & 0.028
\\
Picklock & 80 & 3 & 5 & 5 & 12 & 1 & 0.059 & 1 & 0.058 & 1 & 0.024
\\
Bensalem & 86 & 4 & 4 & 4 & 12 & 1 & 0.058 & 1 & 0.064 & 1 & 0.034
\\
Transfer & 93 & 3 & 10 & 3 & 8 & 0 & 0.048 & 0 & 0.057 & 0 & 0.03
\\
Test & 95 & 3 & 8 & 6 & 14 & 2 & 0.051 & 2 & 0.064 & 2 & 0.026
\\
StringBuffer & 116 & 3 & 14 & 4 & 6 & 2 & 0.053 & 2 & 0.062 & 2 & 0.025
\\
DiningPhil & 398 & 6 & 21 & 6 & 50 & 0 & 0.05 & 1 & 0.074 & 0 & 0.027
\\
HashTable & 522 & 3 & 5 & 3 & 65 & 2 & 0.074 & 2 & 0.078 & 2 & 0.03
\\
DirkAccount & 897 & 6 & 46 & 6 & 72 & 0 & 0.053 & 0 & 0.08 & 0 & 0.027
\\
Log4j2 & 2.47K & 4 & 334 & 11 & 15 & 1 & 0.057 & 1 & 0.066 & 1 & 0.03
\\
Dbcp1 & 2.90K & 3 & 768 & 5 & 14 & 2 & 0.06 & 2 & 0.068 & 2 & 0.031
\\
Derby2 & 3.03K & 3 & 1.01K & 4 & 2 & 1 & 0.077 & 1 & 0.08 & 1 & 0.041
\\
Dbcp2 & 4.09K & 3 & 592 & 10 & 22 & 0 & 0.057 & 0 & 0.083 & 0 & 0.044
\\
JDBCMySQL-1 & 674.54K & 3 & 73.14K & 11 & 4.08K & 2 & 0.273 & 2 & 0.327 & 2 & 0.262
\\
JDBCMySQL-2 & 674.69K & 3 & 73.19K & 11 & 1.28K & 1 & 0.23 & 1 & 0.241 & 1 & 0.289
\\
JDBCMySQL-3 & 675.86K & 3 & 73.25K & 12 & 4.09K & 1 & 0.25 & 1 & 0.343 & 1 & 0.328
\\
JDBCMySQL-4 & 675.99K & 3 & 73.27K & 13 & 4.10K & 2 & 0.308 & 2 & 0.511 & 2 & 0.335
\\
jigsaw-1 & 2.81M & 14 & 63.27K & 105 & 258 & 0 & 0.401 & 0 & 0.612 & 0 & 0.301
\\
jigsaw-2 & 3.20M & 15 & 103.52K & 276 & 1.07K & 0 & 1.628 & 0 & 0.744 & 0 & 0.484
\\
ArrayList & 4.06M & 801 & 120.56K & 802 & 81.42K & 3 & 22.116 & 3 & 1.851 & 3 & 1.609
\\
Stack & 4.43M & 801 & 118.27K & 1.60K & 165.90K & 3 & 20.459 & 3 & 4.189 & 3 & 3.097
\\
IdentityHashMap & 4.55M & 801 & 496.05K & 802 & 80.88K & 1 & 10.123 & 1 & 1.717 & 1 & 1.74
\\
LinkedList & 4.85M & 801 & 289.94K & 802 & 81.35K & 3 & 45.879 & 3 & 2.461 & 3 & 2.051
\\
HashMap & 5.35M & 801 & 554.70K & 802 & 84.64K & 2 & 683.553 & 2 & 1.986 & 2 & 2.036
\\
Vector & 5.40M & 3 & 14 & 3 & 400.00K & 1 & 1.787 & 1 & 2.172 & 1 & 1.17
\\
LinkedHashMap & 6.17M & 801 & 617.02K & 802 & 84.64K & 2 & 556.54 & 2 & 1.893 & 2 & 2.283
\\
WeakHashMap & 6.32M & 801 & 540.35K & 802 & 84.54K & 2 & 695.652 & 2 & 1.864 & 2 & 2.095
\\
montecarlo & 10.13M & 3 & 850.16K & 2 & 4 & 0 & 2.336 & 0 & 0.873 & 0 & 0.786
\\
TreeMap & 19.48M & 801 & 493.45K & 802 & 84.64K & 2 & 655.245 & 2 & 2.965 & 2 & 2.47
\\
hsqldb & 20.00M & 46 & 945.04K & 402 & 167.44K & 0 & - & 0 & 2.482 & 0 & 5.005
\\
sunflow & 34.85M & 16 & 2.03M & 11 & 602 & 0 & 11.095 & 0 & 2.351 & 0 & 2.459
\\
TestPerf-1 & 36.45M & 52 & 623 & 9 & 22.77K & 0 & 11.836 & 0 & 2.361 & 0 & 1.673
\\
tradesoap & 42.03M & 236 & 2.84M & 6.11K & 58.27K & 0 & 92.916 & 0 & 8.317 & 0 & 5.766
\\
tradebeans & 42.04M & 236 & 2.83M & 6.11K & 58.34K & 0 & 92.409 & 0 & 8.3 & 0 & 5.576
\\
jspider & 47.53M & 11 & 4.79M & 15 & 5.23K & 0 & 10.637 & 0 & 3.786 & 0 & 3.615
\\
eclipse & 126.28M & 15 & 10.45M & 4.69K & 161.18K & 0 & 32.867 & 0 & 15.687 & 0 & 10.255
\\
TestPerf-2 & 200.10M & 50 & 599 & 9 & 98.27K & 0 & 54.806 & 0 & 16.026 & 0 & 7.853
\\
Groovy2 & 212.76M & 13 & 12.73M & 9.89K & 10.82K & 0 & 49.639 & 0 & 15.48 & 0 & 13.266
\\
biojava & 221.13M & 6 & 121.02K & 79 & 383 & 0 & 69.125 & 0 & 12.338 & 0 & 13.392
\\
graphchi & 240.66M & 20 & 24.88M & 61 & 344 & 0 & 118.925 & 0 & 21.14 & 0 & 24.955
\\
batik & 279.91M & 7 & 5.11M & 1.92K & 56 & 0 & 17.491 & 0 & 18.094 & 0 & 15.417
\\
\hline
\hline
\textbf{Total} & \textbf{1.58B} & & \textbf{71.27M} & \textbf{37.02K} & \textbf{1.75M} & \textbf{37} & \textbf{3259.326} & \textbf{38} & \textbf{152.072} & \textbf{37} & \textbf{130.991}
\\
\hline
\end{tabular}
}
\end{table*}

